Partitioning Graph Databases - A Quantitative Evaluation

Electronic data is growing at increasing rates, in both size and connectivity: the increasing presence of, and interest in, relationships between data. An example is the Twitter social network graph. Due to this growth demand is increasing for technologies that can process such data. Currently relational databases are the predominant technology, but they are poorly suited to processing connected data as they are optimized for index-intensive operations. Conversely, graph databases are optimized for graph computation. They link records by direct references, avoiding index lookups, and enabling retrieval of adjacent elements in constant time, regardless of graph size. However, as data volume increases these databases outgrow the resources of one computer and data partitioning becomes necessary. We evaluate the viability of using graph partitioning algorithms to partition graph databases. A prototype partitioned database was developed. Three partitioning algorithms explored and one implemented. Three graph datasets were used: two real and one synthetically generated. These were partitioned in various ways and the impact on database performance measured. We defined one synthetic access pattern per dataset and executed each on the partitioned datasets. Evaluation took place in a simulation environment, ensuring repeatability and allowing measurement of metrics like network traffic and load balance. Results show that compared to random partitioning the partitioning algorithm reduced traffic by 40-90%. Executing the algorithm intermittently during usage maintained partition quality, while requiring only 1% the computation of initial partitioning. Strong correlations were found between theoretic quality metrics and generated network traffic under non-uniform access patterns.

==> 03_List_Of_Symbols.tex <==
\chapter{List of Symbols}
%\addcontentsline{toc}{chapter}{List of Symbols}
%\chapter*{List of Abbreviations and Symbols}

\begin{longtable}
{>{\raggedright}p{0.10\textwidth}>{\raggedright}p{0.18\textwidth}>{\raggedright\arraybackslash}p{0.64\textwidth}}
%{>{\raggedright}p{1.5cm}>{\raggedright}p{2.2cm}>{\raggedright\arraybackslash}p{8.5cm}}
  $G$ & \textbf{Simple Graph} & Set of vertices, $V$, and undirected edges, $E$. \linebreak 
  $E \subseteq \lbrace V \times V \rbrace$ 
  \begin{equation}
  G = (V,E) \nonumber
  \end{equation}
  \\ 
  
  $G_P$ & \textbf{Property Graph} & 
  Edges are directed, $E \subseteq ( V \times V )$.
  Edges are labeled, $\lambda : E \rightarrow \Sigma$.
  Properties are a map from keys to values, $\mu : (V \cup E) \times R \rightarrow S$.
  \begin{equation}
  G_P = (V,E,\lambda,\mu) \nonumber  
  \end{equation} 
  \\ 
  
  $e$ & \textbf{Edge} & Connects two vertices, $v$ \mbox{\&} $u$. 
  \begin{equation}
  e=\lbrace v,u \rbrace \nonumber  
  \end{equation} 
  \\ 
  
  $d^{\mathcal{I}}(v)$ & \textbf{In Degree} & Sum of the weights of edges connected to vertex $v$.
  Where $v$ is the destination vertex. 
  \begin{equation}
  d^{\mathcal{I}}(v)= \sum_{e = \lbrace \cdot , v \rbrace \in E} w(e) \nonumber 
  \end{equation} 
  \\ 
  
  $d^{\mathcal{O}}(v)$ & \textbf{Out Degree} & Sum of the weights of edges connected to vertex $v$.
  Where $v$ is the source vertex. 
  \begin{equation}
  d^{\mathcal{O}}(v)= \sum_{e = \lbrace v , \cdot \rbrace \in E} w(e) \nonumber 
  \end{equation} 
  \\ 
  
  $d(v)$ & \textbf{Degree} & Sum of the weights of edges connected to vertex $v$. 
  \begin{equation}
  d(v)= d^{\mathcal{I}}(v) + d^{\mathcal{O}}(v) \nonumber 
  \end{equation} 
  \\ 
  
  $w(e)$ & \textbf{Edge Weight} & Weight value associated with edge $e$. \\ \tabularnewline 
  
  $\pi$ & \textbf{Partition} & Subset of vertices in V. 
  \begin{equation}
  \pi \subseteq V \nonumber 
  \end{equation} 
  \\ 
  
  $\pi^c$ & \textbf{Partition \linebreak Compliment} & 
  All vertices in $V$ that are not in $\pi$. 
  \begin{equation}
  \pi^c = V \setminus \pi \nonumber 
  \end{equation} 
  \\ 
  
  $\Pi$ & \textbf{Partitioning} & Function that divides $V$ into $k$ disjoint subsets. 
  \begin{eqnarray}
  \Pi = V \rightarrow \lbrace \pi_1,\ldots,\pi_k \rbrace \nonumber \\
  V = \pi_1 \cup \pi_2 \cup \ldots \cup \pi_k \nonumber 
  \end{eqnarray} 
  \\ 
  
  $C(\pi_1,\pi_2)$ & \textbf{Connected} & Two partitioned are connected if at least one edge exists between them
  \begin{equation}
  C(\pi_1,\pi_2) \iff
  \exists \lbrace u,v \rbrace \in E \mbox{ ; } ( u \in \pi_1 \wedge v \in \pi_2 ) \nonumber 
  \end{equation}
  \\ 
  
  $\mu(S)$ & \textbf{Volume} & Sum of the degrees of vertices in a set, S. 
  \begin{equation}
  \mu(S) = \sum_{v \in S} d(v) \nonumber 
  \end{equation}
  \\ 
  
  $iw(S)$ & \textbf{Intra-Weight} & Sum of the weights of edges connecting a set of vertices. 
  \begin{equation}
  iw(S)= \sum_{\lbrace u,v \rbrace \in E} w(e) \mbox{ ; } u,v \in S \nonumber
  \end{equation}
  \\ 
  
  $\partial(\pi)$ & \textbf{Partition \linebreak Degree} & Sum of weights of edges leaving $\pi$. 
  \begin{equation}
  \partial(\pi) = ec(\pi,\pi^c) \nonumber 
  \end{equation}
  \\ 
  
  $\delta(\pi)$ & \textbf{Partition \linebreak Boundary} & All vertices on the border of a partition, 
  including those inside and outside of the partition.
  \begin{eqnarray}
  \delta(\pi)_{INNER} & = & 
  \lbrace u \mbox{ ; } u \in \pi \mbox{ } \wedge \mbox{ } ec(\lbrace u \rbrace,\pi^c) > 0 \rbrace \nonumber \\
  \delta(\pi)_{OUTER} & = & 
  \lbrace v \mbox{ ; } v \in \pi^c \mbox{ } \wedge \mbox{ } ec(\lbrace v \rbrace,\pi) > 0 \rbrace \nonumber \\
  \delta(\pi) & = & \delta(\pi)_{INNER} \mbox{ } \cup \mbox{ } \delta(\pi)_{OUTER} \nonumber
  \end{eqnarray}
  \\ 
  
  $ec(G)$ & \textbf{Edge Cut} & Quality measure of a partitioning. Lower values are desirable. 
  \begin{equation}
  ec(G)= \sum^k_{i=1} \left( \sum_{e = \lbrace u,v\rbrace \in E} w(e) \mbox{ ; } 	
  u \in \pi_i \wedge v \not\in \pi_i \right) \nonumber 
  \end{equation}
  \\ 
  
  $ec(\pi_1,\pi_2)$ & \textbf{Edge Cut} & Quality measure of a partitioning. Lower values are desirable. 
  \begin{equation}
  ec(\pi_1,\pi_2)= \sum_{e = \lbrace u,v\rbrace \in E} w(e)
  \mbox{ ; } u \in \pi_1 \wedge v \in \pi_2  \nonumber 
  \end{equation}
  \\ 
  
  $\phi(\pi)$ & \textbf{Conductance} & Quality measure of partitions. Lower values are desirable. 
  \begin{equation}
  \phi(\pi) = \partial(\pi) / \mu(\pi) \nonumber 
  \end{equation}
  \\ 

  $Mod(\Pi)$ & \textbf{Modularity} & Quality measure of a partitioning. Higher values are desirable. 
  \begin{equation}
  Mod(\Pi) = 
  \sum^k_{c=1} \left( \dfrac{iw(\pi_c)}{iw(G)} - 
  \left( \dfrac{\sum_{v\in \pi_c d(v)}}{2iw(G)}\right)^2 \right) \nonumber 
  \end{equation}
  \\ 

  $e^{\mathcal{A}}$ & \textbf{Intra Edge} & An edge, $e=\lbrace u,v \rbrace$, 
  is an intra-edge if it connects two vertices, $u$ and $v$, that belong to the same partition.
  \begin{equation}
  \mbox{intra}( \lbrace u,v \rbrace ) = 
  \begin{cases}
  \mbox{true} & u,v \in \pi_i \\
  \mbox{false} & u \in \pi_i \wedge v \not\in \pi_i
  \end{cases} \nonumber
  \end{equation} 
  \\ 

  $e^{\mathcal{E}}$ & \textbf{Inter Edge} & An edge, $e=\lbrace u,v \rbrace$, 
  is an inter-edge if it connects two vertices, $u$ and $v$, that belong to different partitions.
  \begin{equation}
  \mbox{inter}( \lbrace u,v \rbrace ) = 
  \begin{cases}
  \mbox{true} & u \in \pi_i \wedge v \not\in \pi_i \\
  \mbox{false} & u,v \in \pi_i
  \end{cases} \nonumber
  \end{equation} 
  \\ 

%  $intra(e)$ & \textbf{Intra Edge} & Edge that connects vertices belonging to the same partition.
%  \begin{equation}
%  intra( \lbrace u,v \rbrace ) = 
%  \begin{cases}
%  \mbox{true} & u,v \in \pi_i \nonumber \\
%  \mbox{false} & u \in \pi_i \wedge v \not\in \pi_i
%  \end{cases} \nonumber
%  \end{equation} 
%  \\ 
%
%  $inter(e)$ & \textbf{Inter Edge} & Edge that connects vertices belonging to different partitions.
%  \begin{equation}
%  inter( \lbrace u,v \rbrace ) = 
%  \begin{cases}
%  \mbox{true} & u \in \pi_i \wedge v \not\in \pi_i \\
%  \mbox{false} & u,v \in \pi_i
%  \end{cases} \nonumber
%  \end{equation} 
%  \\ 
  
%  $ie(e)$ & \textbf{Intra Edge} & An edge $e={v,u}$ is an intra edge if $v,u \in \pi_i $  \\  
%  
%  $oe(e)$ & \textbf{Inter Edge} & An edge $e={v,u}$ is an intra edge if $v \in \pi_i, u \in \pi_j, \pi_i \neq \pi_j $ \\
\end{longtable}
